Exploiting the Natural Dynamics of Series Elastic Robots by Actuator-Centered Sequential Linear Programming

Series elastic robots are best able to follow trajectories which obey the limitations of their actuators, since they cannot instantly change their joint forces. In fact, the performance of series elastic actuators can surpass that of ideal force source actuators by storing and releasing energy. In this paper, we formulate the trajectory optimization problem for series elastic robots in a novel way based on sequential linear programming. Our framework is unique in the separation of the actuator dynamics from the rest of the dynamics, and in the use of a tunable pseudo-mass parameter that improves the discretization accuracy of our approach. The actuator dynamics are truly linear, which allows them to be excluded from trust-region mechanics. This causes our algorithm to have similar run times with and without the actuator dynamics. We demonstrate our optimization algorithm by tuning high performance behaviors for a single-leg robot in simulation and on hardware for a single degree-of-freedom actuator testbed. The results show that compliance allows for faster motions and takes a similar amount of computation time.

==> bib.tex <==
@inproceedings{chen2013optimal,
  title={Optimal control for maximizing velocity of the CompAct™ compliant actuator},
  author={Chen, Lisha and Garabini, Manolo and Laffranchi, Matteo and Kashiri, Navvab and Tsagarakis, Nikos G and Bicchi, Antonio and Caldwell, Darwin G},
  booktitle={Robotics and Automation (ICRA), 2013 IEEE International Conference on},
  pages={516--522},
  year={2013},
  organization={IEEE}
}

@inproceedings{pratt1995series,
  title={Series elastic actuators},
  author={Pratt, Gill A and Williamson, Matthew M},
  booktitle={Intelligent Robots and Systems 95. `Human Robot Interaction and Cooperative Robots', Proceedings. 1995 IEEE/RSJ International Conference on},
  volume={1},
  pages={399--406},
  year={1995},
  organization={IEEE}
}

@article{paine2014design,
  title={Design and control considerations for high-performance series elastic actuators},
  author={Paine, Nicholas and Oh, Sehoon and Sentis, Luis},
  journal={IEEE/ASME Transactions on Mechatronics},
  volume={19},
  number={3},
  pages={1080--1091},
  year={2014},
  publisher={IEEE}
}

@inproceedings{orekhov2015unlumped,
  title={An unlumped model for linear series elastic actuators with ball screw drives},
  author={Orekhov, Viktor L and Knabe, Coleman S and Hopkins, Michael A and Hong, Dennis W},
  booktitle={Intelligent Robots and Systems (IROS), 2015 IEEE/RSJ International Conference on},
  pages={2224--2230},
  year={2015},
  organization={IEEE}
}

@inproceedings{schutz2016intuitive,
  title={An intuitive and comprehensive two-load model for Series Elastic Actuators},
  author={Sch{\"u}tz, Steffen and Nejadfard, Atabak and K{\"o}tting, Christian and Berns, Karsten},
  booktitle={Advanced Motion Control (AMC), 2016 IEEE 14th International Workshop on},
  pages={573--580},
  year={2016},
  organization={IEEE}
}

@inproceedings{ito2014development,
  title={Development and verification of life-size humanoid with high-output actuation system},
  author={Ito, Yoshito and Nozawa, Shunich and Urata, Junichi and Nakaoka, Takuya and Kobayashi, Kazuya and Nakanishi, Yuto and Okada, Kei and Inaba, Masayuki},
  booktitle={Robotics and Automation (ICRA), 2014 IEEE International Conference on},
  pages={3433--3438},
  year={2014},
  organization={IEEE}
}

@misc{cvx,
  author       = {Michael Grant and Stephen Boyd},
  title        = {{CVX}: Matlab Software for Disciplined Convex Programming, version 2.1},
  month        = mar,
  year         = 2014
}


@inproceedings{li2004iterative,
  title={Iterative linear quadratic regulator design for nonlinear biological movement systems.},
  author={Li, Weiwei and Todorov, Emanuel},
  booktitle={ICINCO (1)},
  pages={222--229},
  year={2004}
}

@article{tedrake2010lqr,
  title={LQR-trees: Feedback motion planning via sums-of-squares verification},
  author={Tedrake, Russ and Manchester, Ian R and Tobenkin, Mark and Roberts, John W},
  journal={The International Journal of Robotics Research},
  volume={29},
  number={8},
  pages={1038--1052},
  year={2010},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{todorov2005generalized,
  title={A generalized iterative LQG method for locally-optimal feedback control of constrained nonlinear stochastic systems},
  author={Todorov, Emanuel and Li, Weiwei},
  booktitle={American Control Conference, 2005. Proceedings of the 2005},
  pages={300--306},
  year={2005},
  organization={IEEE}
}

@inproceedings{schulman2013finding,
  title={Finding Locally Optimal, Collision-Free Trajectories with Sequential Convex Optimization.},
  author={Schulman, John and Ho, Jonathan and Lee, Alex X and Awwal, Ibrahim and Bradlow, Henry and Abbeel, Pieter},
  booktitle={Robotics: science and systems},
  volume={9},
  number={1},
  pages={1--10},
  year={2013}
}

@inproceedings{ThomasSentis2016IROS,
  title={Towards computationally efficient planning of dynamic multi-contact locomotion},
  author={Thomas, Gray C and Sentis, Luis},
  booktitle={Intelligent Robots and Systems (IROS), 2016 IEEE/RSJ International Conference on},
  pages={3879--3886},
  year={2016},
  organization={IEEE}
}

@article{betts1998survey,
  title={Survey of numerical methods for trajectory optimization},
  author={Betts, John T},
  journal={Journal of Guidance control and dynamics},
  volume={21},
  number={2},
  pages={193--207},
  year={1998},
  publisher={New York: The Institute, 1982-}
}

@article{haddadin2011optimal,
  title={Optimal control for maximizing link velocity of robotic variable stiffness joints},
  author={Haddadin, Sami and Weis, Michael and Wolf, Sebastian and Albu-Sch{\"a}ffer, Alin},
  journal={IFAC Proceedings Volumes},
  volume={44},
  number={1},
  pages={6863--6871},
  year={2011},
  publisher={Elsevier}
}

@article{braun2012optimal,
  title={Optimal variable stiffness control: formulation and application to explosive movement tasks},
  author={Braun, David and Howard, Matthew and Vijayakumar, Sethu},
  journal={Autonomous Robots},
  volume={33},
  number={3},
  pages={237--253},
  year={2012},
  publisher={Springer}
}

@article{braun2013robots,
  title={Robots driven by compliant actuators: Optimal control under actuation constraints},
  author={Braun, David J and Petit, Florian and Huber, Felix and Haddadin, Sami and Van Der Smagt, Patrick and Albu-Sch{\"a}ffer, Alin and Vijayakumar, Sethu},
  journal={IEEE Transactions on Robotics},
  volume={29},
  number={5},
  pages={1085--1101},
  year={2013},
  publisher={IEEE}
}

@inproceedings{radulescu2012exploiting,
  title={Exploiting variable physical damping in rapid movement tasks},
  author={Radulescu, Andreea and Howard, Matthew and Braun, David J and Vijayakumar, Sethu},
  booktitle={Advanced Intelligent Mechatronics (AIM), 2012 IEEE/ASME International Conference on},
  pages={141--148},
  year={2012},
  organization={IEEE}
}

@inproceedings{garabini2011optimality,
  title={Optimality principles in variable stiffness control: The vsa hammer},
  author={Garabini, Manolo and Passaglia, Andrea and Belo, Felipe and Salaris, Paolo and Bicchi, Antonio},
  booktitle={Intelligent Robots and Systems (IROS), 2011 IEEE/RSJ International Conference on},
  pages={3770--3775},
  year={2011},
  organization={IEEE}
}

@inproceedings{ito2010development,
  title={Development of very small high output motor driver for realizing forceful musculoskeletal humanoids},
  author={Ito, Nobuyuki and Urata, Junichi and Nakanishi, Yuto and Okada, Kei and Inaba, Masayuki},
  booktitle={Humanoid Robots (Humanoids), 2010 10th IEEE-RAS International Conference on},
  pages={385--390},
  year={2010},
  organization={IEEE}
}

@inproceedings{urata2010design,
  title={Design of high torque and high speed leg module for high power humanoid},
  author={Urata, Junichi and Nakanishi, Yuto and Okada, Kei and Inaba, Masayuki},
  booktitle={Intelligent Robots and Systems (IROS), 2010 IEEE/RSJ International Conference on},
  pages={4497--4502},
  year={2010},
  organization={IEEE}
}

@article{grizzle20103d,
  title={{3D} bipedal robotic walking: models, feedback control, and open problems},
  author={Grizzle, Jessy W and Chevallereau, Christine and Ames, Aaron D and Sinnet, Ryan W},
  journal={IFAC Proceedings Volumes},
  volume={43},
  number={14},
  pages={505--532},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{haddadin2012optimal,
  title={Optimal control for exploiting the natural dynamics of variable stiffness robots},
  author={Haddadin, Sami and Huber, Felix and Albu-Sch{\"a}ffer, Alin},
  booktitle={Robotics and Automation (ICRA), 2012 IEEE International Conference on},
  pages={3347--3354},
  year={2012},
  organization={IEEE}
}

@book{al05,
author = {Harry Asada and John Leonard},
publisher = {Fall Massachusetts Institute of Technology: MIT OpenCourseWare, License: Creative Commons BY-NC-SA},
title = {2.12 Introduction to Robotics},
year = {2005},
url = {https://ocw.mit.edu},
}

@inproceedings{werner2014trajectory,
  title={Trajectory optimization for walking robots with series elastic actuators},
  author={Werner, Alexander and Lampariello, Roberto and Ott, Christian},
  booktitle={Decision and Control (CDC), 2014 IEEE 53rd Annual Conference on},
  pages={2964--2970},
  year={2014},
  organization={IEEE}
}

@article{sreenath2011compliant,
  title={A compliant hybrid zero dynamics controller for stable, efficient and fast bipedal walking on {MABEL}},
  author={Sreenath, Koushil and Park, Hae-Won and Poulakakis, Ioannis and Grizzle, Jessy W},
  journal={The International Journal of Robotics Research},
  volume={30},
  number={9},
  pages={1170--1193},
  year={2011},
  publisher={Sage Publications Sage UK: London, England}
}

@article{meirovitch1995trajectory,
  title={Trajectory and control optimization for flexible space robots},
  author={Meirovitch, L and Chen, Y},
  journal={Journal of Guidance, Control, and Dynamics},
  volume={18},
  number={3},
  pages={493--502},
  year={1995}
}

@inproceedings{ratliff2009chomp,
  title={CHOMP: Gradient optimization techniques for efficient motion planning},
  author={Ratliff, Nathan and Zucker, Matt and Bagnell, J Andrew and Srinivasa, Siddhartha},
  booktitle={Robotics and Automation, 2009. ICRA'09. IEEE International Conference on},
  pages={489--494},
  year={2009},
  organization={IEEE}
}

@inproceedings{moro2011human,
  title={A human-like walking for the {CO}mpliant hu{MAN}oid {COMAN} based on {CoM} trajectory reconstruction from kinematic Motion Primitives},
  author={Moro, Federico L and Tsagarakis, Nikos G and Caldwell, Darwin G},
  booktitle={Humanoid Robots (Humanoids), 2011 11th IEEE-RAS International Conference on},
  pages={364--370},
  year={2011},
  organization={IEEE}
}

@article{sreenath2013embedding,
  title={Embedding active force control within the compliant hybrid zero dynamics to achieve stable, fast running on {MABEL}},
  author={Sreenath, Koushil and Park, Hae-Won and Poulakakis, Ioannis and Grizzle, Jessy W},
  journal={The International Journal of Robotics Research},
  volume={32},
  number={3},
  pages={324--345},
  year={2013},
  publisher={SAGE Publications Sage UK: London, England}
}

@inproceedings{hereid20163d,
  title={{3D} dynamic walking with underactuated humanoid robots: A direct collocation framework for optimizing hybrid zero dynamics},
  author={Hereid, Ayonga and Cousineau, Eric A and Hubicki, Christian M and Ames, Aaron D},
  booktitle={Robotics and Automation (ICRA), 2016 IEEE International Conference on},
  pages={1447--1454},
  year={2016},
  organization={IEEE}
}

@inproceedings{werner2012optimization,
  title={Optimization-based generation and experimental validation of optimal walking trajectories for biped robots},
  author={Werner, Alexander and Lampariello, Roberto and Ott, Christian},
  booktitle={Intelligent Robots and Systems (IROS), 2012 IEEE/RSJ International Conference on},
  pages={4373--4379},
  year={2012},
  organization={IEEE}
}

@article{pratt2012capturability,
  title={Capturability-based analysis and control of legged locomotion, Part 2: Application to M2V2, a lower-body humanoid},
  author={Pratt, Jerry and Koolen, Twan and De Boer, Tomas and Rebula, John and Cotton, Sebastien and Carff, John and Johnson, Matthew and Neuhaus, Peter},
  journal={The International Journal of Robotics Research},
  volume={31},
  number={10},
  pages={1117--1133},
  year={2012},
  publisher={SAGE Publications Sage UK: London, England}
}

@misc{Schlossman2017,
  author = {Schlossman, Rachel},
  title = {},
  year = {2018},
  publisher = {GitHub},
  journal = {GitHub repository},
  howpublished = {\url{https://github.com/rschloss123}},
  commit = {}
}

@inproceedings{werner2017generation,
  title={Generation of Locomotion Trajectories for Series Elastic and Viscoelastic Bipedal Robots},
  author={Werner, Alexander and Turlej, Wojciech and Ott, Christian},
  booktitle={IEEE International Conference on Intelligent Robots and Systems},
  year={2017}
}

 @misc{gurobi,
   author = "Gurobi Optimization, Inc.",
   title = "Gurobi Optimizer Reference Manual",
   year = 2016,
   url = "http://www.gurobi.com"
 }
 
 @article{vanderborght2013variable,
  title={Variable impedance actuators: A review},
  author={Vanderborght, Bram and Albu-Sch{\"a}ffer, Alin and Bicchi, Antonio and Burdet, Etienne and Caldwell, Darwin G and Carloni, Raffaella and Catalano, M and Eiberger, Oliver and Friedl, Werner and Ganesh, Ganesh and others},
  journal={Robotics and autonomous systems},
  volume={61},
  number={12},
  pages={1601--1614},
  year={2013},
  publisher={Elsevier}
}

@article{koolen2016design,
  title={Design of a momentum-based control framework and application to the humanoid robot atlas},
  author={Koolen, Twan and Bertrand, Sylvain and Thomas, Gray and De Boer, Tomas and Wu, Tingfan and Smith, Jesper and Englsberger, Johannes and Pratt, Jerry},
  journal={International Journal of Humanoid Robotics},
  volume={13},
  number={01},
  pages={1650007},
  year={2016},
  publisher={World Scientific}
}

@article{giftthaler2018control,
  title={The Control Toolbox-An Open-Source C++ Library for Robotics, Optimal and Model Predictive Control},
  author={Giftthaler, Markus and Neunert, Michael and St{\"a}uble, Markus and Buchli, Jonas},
  journal={arXiv preprint arXiv:1801.04290},
  year={2018}
}

@inproceedings{thomas2016towards,
  title={Towards computationally efficient planning of dynamic multi-contact locomotion},
  author={Thomas, Gray C and Sentis, Luis},
  booktitle={Intelligent Robots and Systems (IROS), 2016 IEEE/RSJ International Conference on},
  pages={3879--3886},
  year={2016},
  organization={IEEE}
}

@inproceedings{werner2017optimal,
  title={Optimal and Robust Walking using Intrinsic Properties of a Series-Elastic Robot},
  author={Werner, Alexander and Henze, Bernd and Loeffl, Florian Christoph and Leyendecker, Sigrid and Ott, Christian},
  booktitle={IEEE-RAS International Conference on Humanoid Robots},
  year={2017}
}

@inproceedings{kwak2017comparison,
  title={Comparison of resonance ratio control and inner force control for series elastic actuator},
  author={Kwak, Su Hui and Oh, Sehoon},
  booktitle={Industrial Electronics Society, IECON 2017-43rd Annual Conference of the IEEE},
  pages={7583--7588},
  year={2017},
  organization={IEEE}
}

@article{cvxpy,
  author  = {Steven Diamond and Stephen Boyd},
  title   = {{CVXPY}: A {P}ython-Embedded Modeling Language for Convex Optimization},
  journal = {Journal of Machine Learning Research},
  year    = {2016},
  volume  = {17},
  number  = {83},
  pages   = {1--5},
}
